Exploiting Sparsity in Automotive Radar Object Detection Networks

Having precise perception of the environment is crucial for ensuring the secure and reliable functioning of autonomous driving systems. Radar object detection networks are one fundamental part of such systems. CNN-based object detectors showed good performance in this context, but they require large compute resources. This paper investigates sparse convolutional object detection networks, which combine powerful grid-based detection with low compute resources. We investigate radar specific challenges and propose sparse kernel point pillars (SKPP) and dual voxel point convolutions (DVPC) as remedies for the grid rendering and sparse backbone architectures. We evaluate our SKPP-DPVCN architecture on nuScenes, which outperforms the baseline by 5.89% and the previous state of the art by 4.19% in Car AP4.0. Moreover, SKPP-DPVCN reduces the average scale error (ASE) by 21.41% over the baseline.

==> saved_sections.tex <==
\subsection{Submanifold Sparse Kernel Point Convolution Backbone}
The original PointPillars Backbone processes a dense pseudoimage with a convolutional feature pyramid network backbone\cite{Lin_2017_CVPR}. Our empirical findings indicate that this backbone architecture exhibits poor performance when applied to radar data, which aligns with the observations made in \cite{scheiner_object_2021}. In addition, this network is not capable of processing sparse grid representations. Instead, we use a Submanifold sparse U-Net (SSCN) as backbone, which is described in detail in \cite{graham20173d}. As in the original paper, the SSCN uses a sparse voxelized inut representation, which can be the result of the sparse PointPillar or our SKPP grid-rendering module. We denote a sparse convolution SC($m$,$n$,$f$,$s$) with $m$ input feature planes, $n$ output feature planes, a filter size of $f$ and stride $s$. Like in the original paper, a submanifold sparse convolution SSC( $m$,$n$,$f$) is a modified SC($m$,$n$,$f$,$s=1$). The original SSCNs basic building block consists out of two "pre-activated" SSC(.,.,3) convolutions which are preceded by batch normalization ad a ReLU non-linearity. SC(·, ·, 2, 2) convolutions are utilized whenever the networks downsamples the spatial scale by a factor of two. We use deconvolution operations DC(.,.,$f$,$s$) to "invert" the SC(·, ·, 2, 2) convolutions. The active output sites in a DC convolution are identical to the active input sites in the corresponding SC convolution. The connections between input and output sites are merely reversed. For further details, we refer to \cite{deconv}. However, the submanifold sparse convolution layer processes the environment with a kernel size of 3, neglecting the distance to the surrounding points and thus not taking into account the spatial information at different scaling levels. To also preserve spatial information within the reduced spatial scaling of SSCN, we introduce submanifold sparse kernel point convolution (SSKPCN) and use the descriptive power of KPConv within a block of the U-Net. Fig \ref{fig: backbone_architecture} illustrates the U-Net architecture. We we have noticed that it is beneficial to use additional kpconv layers only during the encoder block. The number of the KPConv blocks are equaly to the number of conv blocks. Each KPConv block in our network consists of a sequence of layers: a Conv1D layer followed by Batch Normalization, a KPConv layer, another Batch Normalization layer, an activation function, and finally another Conv1D layer. Each encoder stage receives the downsampled feature map and performs two sets of conv blocks and two sets of KPConv blocks. Subsequently, the resulting feature maps are normalized using L2 normalization and then added together.  All architectures share the same feature pyramid network \cite{Lin_2017_CVPR} which is similar to \cite{DBLP:journals/corr/abs-1902-06326}. Ultimately, convolutional detection heads and non-maximum suppression (NMS) techniques are employed to produce and refine oriented bounding boxes (OBBs) for various class categories.
